SparQ Attention: Bandwidth-Efficient LLM Inference

The computational difficulties of large language model (LLM) inference remain a significant obstacle to their widespread deployment. The need for many applications to support long input sequences and process them in large batches typically causes token-generation to be bottlenecked by data transfer. For this reason, we introduce SparQ Attention, a technique for increasing the inference throughput of LLMs by utilising memory bandwidth more efficiently within the attention layers, through selective fetching of the cached history. Our proposed technique can be applied directly to off-the-shelf LLMs during inference, without requiring any modification to the pre-training setup or additional fine-tuning. We show that SparQ Attention brings up to 8x savings in attention data transfers without substantial drops in accuracy, by evaluating Llama 2 and 3, Mistral, Gemma and Pythia models on a wide range of downstream tasks.

==> algorithms/old_code.tex <==
% red (strings): 186,34,32
% black (variables): 33,33,33
% purple (operators): 170,35,255
% green (keywords and python built-in functions): 0,128,0
% green (comments): 64,128,128
% blue (type built-in functions): 0,85,170
% grey (cell background): 245,245,246
% grey (cell border): 224, 224, 224

\definecolor{str}{RGB}{186,34,32}
\definecolor{var}{RGB}{33,33,33}
\definecolor{ops}{RGB}{170,35,255}
\definecolor{big}{RGB}{0,128,0}
\definecolor{com}{RGB}{64,128,128}
\definecolor{bib}{RGB}{0,85,170}
\definecolor{fun}{RGB}{0,20,255}

\newcommand{\ccolor}[2]{\textcolor{#1}{#2}}



\small{\fontseries{m}\selectfont\texttt{\ccolor{big}{from} torch \ccolor{big}{import} \codegreen{abs}, \codegreen{softmax}, \codegreen{sqrt}, \codegreen{tensor}, \codegreen{topk}\\[2em]
\ccolor{big}{def} \ccolor{fun}{gather}(t, dim, i):\\
\codetab dim \ccolor{ops}{+=} (dim \ccolor{ops}{<} \ccolor{big}{0}) \ccolor{ops}{*} t.\ccolor{bib}{ndim}\\
\codetab \ccolor{big}{return} t.\ccolor{bib}{gather}(dim, i.\ccolor{bib}{expand}(\ccolor{big}{*}t.\ccolor{bib}{shape}[:dim], i.\ccolor{bib}{shape}[dim], \ccolor{\big}{*}t.\ccolor{bib}{shape}[dim \ccolor{ops}{+} \ccolor{big}{1}:]))\\[2em]
\ccolor{big}{def} \ccolor{fun}{attn}(Q, K, V, M):\\
\codetab s \ccolor{ops}{=} (Q \ccolor{ops}{@} K.\ccolor{bib}{transpose}(\ccolor{ops}{-}\ccolor{big}{1}, \ccolor{ops}{-}\ccolor{big}{2})) \ccolor{ops}{/} sqrt(tensor(Q.\ccolor{bib}{shape}[\ccolor{ops}{-}\ccolor{big}{1}])) \ccolor{ops}{+} M\\
\codetab \ccolor{big}{return} softmax(s, dim\ccolor{ops}{=-}\ccolor{big}{1}) \ccolor{ops}{@} V\\[2em]
\ccolor{big}{def} \ccolor{fun}{sparq\_attn}(Q, K, V, V\_mean, M, r, k):\\
\codetab \textit{\ccolor{com}{\# 1. Approximate attention scores using r largest components of Q}}\\
\codetab i1 \ccolor{ops}{=} topk(abs(Q), r, \ccolor{ops}{-}\ccolor{big}{1}).\ccolor{bib}{indices}\\
\codetab Q\_hat, K\_hat \ccolor{ops}{=} gather(Q, \ccolor{ops}{-}\ccolor{big}{1}, i1), \codeblue{gather}(K, \ccolor{ops}{-}\ccolor{big}{1}, i1)\\
\codetab scale \ccolor{ops}{=} sqrt(\\
\codetab\codetab Q.\ccolor{bib}{shape}[\ccolor{ops}{-}\ccolor{big}{1}]\\
\codetab\codetab \ccolor{ops}{*} abs(Q\_hat).sum(dim\ccolor{ops}{=-}\ccolor{big}{1}, keepdim\ccolor{ops}{=}\ccolor{big}{True})\\
\codetab\codetab \ccolor{ops}{/} abs(Q).sum(dim\ccolor{ops}{=-}\ccolor{big}{1}, keepdim\ccolor{ops}{=}\ccolor{big}{True})\\
\codetab )\\
\codetab s\_hat \ccolor{ops}{=} softmax(Q\_hat \ccolor{ops}{@} K\_hat.\ccolor{bib}{transpose}(\ccolor{ops}{-}\ccolor{big}{1}, \ccolor{ops}{-}\ccolor{big}{2}) \ccolor{ops}{/} scale \ccolor{ops}{+} M, dim\ccolor{ops}{=-}\ccolor{big}{1})\\[1em]
\codetab \textit{\ccolor{com}{\# 2. Gather top-k positions based on approximate attention scores and run attention}}\\
\codetab i2 \ccolor{ops}{=} topk(s\_hat, k, \ccolor{ops}{-}\ccolor{big}{1}).\ccolor{bib}{indices}\\
\codetab iKV \ccolor{ops}{=} i2[\ccolor{bib}{...}, \ccolor{big}{0}, :, \ccolor{big}{None}]\\
\codetab K, V, M \ccolor{ops}{=} gather(K, \ccolor{ops}{-}\ccolor{big}{1}, iKV), gather(V, \ccolor{ops}{-}\ccolor{big}{2}, iKV), gather(M, \ccolor{ops}{-}\ccolor{big}{1}, i2)\\
\codetab y\_ \ccolor{ops}{=} \codeblue{attn}(Q, K, V, M)\\[1em]
\codetab \textit{\ccolor{com}{\# 3. Estimate the total score of the top-k, and interpolate with V\_mean}}\\
\codetab alpha \ccolor{ops}{=} gather(s\_hat, \ccolor{ops}{-}\ccolor{big}{1}, i2).\ccolor{bib}{sum}(\ccolor{ops}{-}\ccolor{big}{1}, keepdim\ccolor{ops}{=}\ccolor{big}{True})\\
\codetab \ccolor{big}{return} alpha \ccolor{ops}{*} y\_ \ccolor{ops}{+} (\ccolor{big}{1} \ccolor{ops}{-} alpha) \ccolor{ops}{*} V\_mean}}


==> figures/sparq_schematic.tex <==
%auto-ignore

\begin{tikzpicture}

% Sparse Query
\fill[fill=none] (-1, 0) rectangle (0, 1) node[pos=0.5] {\LARGE $\bm{q}_{[\textcolor{gc_dark_pink}{\bm{i}_1}]}$};
\filldraw[draw=black, fill=gc_pink] (2, 0) rectangle (3, 1) node[pos=0.5] {$\bm{0.8}$};
\filldraw[draw=black, fill=gc_gray] (3, 0) rectangle (4, 1) node[pos=0.5] {$-0.2$};
\filldraw[draw=black, fill=gc_pink] (4, 0) rectangle (5, 1) node[pos=0.5] {$\bm{-1.3}$};
\filldraw[draw=black, fill=gc_gray] (5, 0) rectangle (6, 1) node[pos=0.5] {$0.4$};
\fill[fill=none] (0.5, 0) rectangle (1.5, 1) node[pos=0.5] {\large \texttt{called}};

\fill[fill=none] (2, 0) rectangle (6, -1) node[pos=0.5] {\LARGE $\bm{\otimes}$};

% Input Sequence
\fill[fill=none] (-1, -1) rectangle (0, -2) node[pos=0.5] {\LARGE $\bm{K}_{[:, \textcolor{gc_dark_pink}{\bm{i}_1}]}$};
\fill[fill=none] (0.5, -1) rectangle (1.5, -2) node[pos=0.5] {\large \texttt{the}};
\fill[fill=none] (0.5, -2) rectangle (1.5, -3) node[pos=0.5] {\large \texttt{dog}};
\fill[fill=none] (0.5, -3) rectangle (1.5, -4) node[pos=0.5] {\large \texttt{ran}};
\fill[fill=none] (0.5, -4) rectangle (1.5, -5) node[pos=0.5] {\large \texttt{towards}};
\fill[fill=none] (0.5, -5) rectangle (1.5, -6) node[pos=0.5] {\large \texttt{the}};
\fill[fill=none] (0.5, -6) rectangle (1.5, -7) node[pos=0.5] {\large \texttt{tree}};
\fill[fill=none] (0.5, -7) rectangle (1.5, -8) node[pos=0.5] {\large \texttt{as}};
\fill[fill=none] (0.5, -8) rectangle (1.5, -9) node[pos=0.5] {\large \texttt{the}};
\fill[fill=none] (0.5, -9) rectangle (1.5, -10) node[pos=0.5] {\large \texttt{owner}};
\fill[fill=none] (0.5, -10) rectangle (1.5, -11) node[pos=0.5] {\large \texttt{called}};

% Key Tensor Colouring
\fill[fill=gc_pink] (2, -1) rectangle (3, -11) node[pos=0.5] {};
\fill[fill=gc_gray] (3, -1) rectangle (4, -11) node[pos=0.5] {};
\fill[fill=gc_pink] (4, -1) rectangle (5, -11) node[pos=0.5] {};
\fill[fill=gc_gray] (5, -1) rectangle (6, -11) node[pos=0.5] {};

% Empty Key Tensor
\filldraw[draw=black, fill=none] (2, -1) rectangle (6, -11) node[pos=0.5] {};
\draw (3, -1) to (3, -11);
\draw (4, -1) to (4, -11);
\draw (5, -1) to (5, -11);
\draw (2, -2) to (6, -2);
\draw (2, -3) to (6, -3);
\draw (2, -4) to (6, -4);
\draw (2, -5) to (6, -5);
\draw (2, -6) to (6, -6);
\draw (2, -7) to (6, -7);
\draw (2, -8) to (6, -8);
\draw (2, -9) to (6, -9);
\draw (2, -10) to (6, -10);


\draw[thick, -Triangle, color=black] (6.25, -6) -- (7.25, -6);


% Approximate Attention Scores
\fill[fill=none] (7.5, 0.8) rectangle (9, 0.4) node[pos=0.5] {\Large approximate};
\fill[fill=none] (7.5, 0.4) rectangle (9, 0) node[pos=0.5] {\Large attention};
\fill[fill=none] (7.5, -0.1) rectangle (9, -0.45) node[pos=0.5] {\Large scores $\bm{\hat{s}}$};


\filldraw[draw=black, fill=gc_gray, dashed] (9, -1) rectangle (8.6, -2) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (9, -2) rectangle (7.6, -3) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (9, -3) rectangle (8.0, -4) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_gray, dashed] (9, -4) rectangle (8.6, -5) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_gray, dashed] (9, -5) rectangle (8.9, -6) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (9, -6) rectangle (7.8, -7) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_gray, dashed] (9, -7) rectangle (8.6, -8) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_gray, dashed] (9, -8) rectangle (8.8, -9) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (9, -9) rectangle (8.0, -10) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_gray, dashed] (9, -10) rectangle (8.4, -11) node[pos=0.5] {};
\draw (9, -0.75) to (9, -11.25);


\draw[thick, -Triangle, color=black] (9.25, -6) -- (11.25, -6);





% Sparse Query
\fill[fill=none] (10, 0) rectangle (11, 1) node[pos=0.5] {\LARGE $\bm{q}$};
\filldraw[draw=black, fill=gc_dark_gray] (11.5, 0) rectangle (12.5, 1) node[pos=0.5] {$0.8$};
\filldraw[draw=black, fill=gc_dark_gray] (12.5, 0) rectangle (13.5, 1) node[pos=0.5] {$-0.2$};
\filldraw[draw=black, fill=gc_dark_gray] (13.5, 0) rectangle (14.5, 1) node[pos=0.5] {$-1.3$};
\filldraw[draw=black, fill=gc_dark_gray] (14.5, 0) rectangle (15.5, 1) node[pos=0.5] {$0.4$};

\fill[fill=none] (11.5, 0) rectangle (15.5, -1) node[pos=0.5] {\LARGE $\bm{\otimes}$};


% Key Tensor Colouring
\fill[fill=gc_gray] (11.5, -1) rectangle (15.5, -2) node[pos=0.5] {};
\fill[fill=gc_blue] (11.5, -2) rectangle (15.5, -3) node[pos=0.5] {};
\fill[fill=gc_blue] (11.5, -3) rectangle (15.5, -4) node[pos=0.5] {};
\fill[fill=gc_gray] (11.5, -4) rectangle (15.5, -5) node[pos=0.5] {};
\fill[fill=gc_gray] (11.5, -5) rectangle (15.5, -6) node[pos=0.5] {};
\fill[fill=gc_blue] (11.5, -6) rectangle (15.5, -7) node[pos=0.5] {};
\fill[fill=gc_gray] (11.5, -7) rectangle (15.5, -8) node[pos=0.5] {};
\fill[fill=gc_gray] (11.5, -8) rectangle (15.5, -9) node[pos=0.5] {};
\fill[fill=gc_blue] (11.5, -9) rectangle (15.5, -10) node[pos=0.5] {};
\fill[fill=gc_gray] (11.5, -10) rectangle (15.5, -11) node[pos=0.5] {};

% Empty Key Tensor
\fill[fill=none] (10, -1) rectangle (11, -2) node[pos=0.5] {\LARGE $\bm{K}_{[\textcolor{gc_dark_blue}{\bm{i}_2}, :]}$};
\filldraw[draw=black, fill=none] (11.5, -1) rectangle (15.5, -11) node[pos=0.5] {};
\draw (12.5, -1) to (12.5, -11);
\draw (13.5, -1) to (13.5, -11);
\draw (14.5, -1) to (14.5, -11);
\draw (11.5, -2) to (15.5, -2);
\draw (11.5, -3) to (15.5, -3);
\draw (11.5, -4) to (15.5, -4);
\draw (11.5, -5) to (15.5, -5);
\draw (11.5, -6) to (15.5, -6);
\draw (11.5, -7) to (15.5, -7);
\draw (11.5, -8) to (15.5, -8);
\draw (11.5, -9) to (15.5, -9);
\draw (11.5, -10) to (15.5, -10);


\draw[thick, -Triangle, color=black] (15.75, -6) -- (16.75, -6);


% Sparse Attention Scores
\fill[fill=none] (17, 0.8) rectangle (18.5, 0.4) node[pos=0.5] {\Large sparse};
\fill[fill=none] (17, 0.4) rectangle (18.5, 0) node[pos=0.5] {\Large attention};
\fill[fill=none] (17, -0.1) rectangle (18.5, -0.45) node[pos=0.5] {\Large scores $\bm{s}$};

\draw (18.5, -0.75) to (18.5, -11.25);
\filldraw[draw=black, fill=gc_dark_gray] (18.5, -2) rectangle (16.8, -3) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (18.5, -3) rectangle (17.8, -4) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (18.5, -6) rectangle (17.1, -7) node[pos=0.5] {};
\filldraw[draw=black, fill=gc_dark_gray] (18.5, -9) rectangle (17.3, -10) node[pos=0.5] {};



\fill[fill=none] (18.5, -1) rectangle (21, -11) node[pos=0.5] {\LARGE $\bm{\otimes}$};


% Value Tensor Colouring
\fill[fill=gc_gray] (21, -1) rectangle (25, -2) node[pos=0.5] {};
\fill[fill=gc_blue] (21, -2) rectangle (25, -3) node[pos=0.5] {};
\fill[fill=gc_blue] (21, -3) rectangle (25, -4) node[pos=0.5] {};
\fill[fill=gc_gray] (21, -4) rectangle (25, -5) node[pos=0.5] {};
\fill[fill=gc_gray] (21, -5) rectangle (25, -6) node[pos=0.5] {};
\fill[fill=gc_blue] (21, -6) rectangle (25, -7) node[pos=0.5] {};
\fill[fill=gc_gray] (21, -7) rectangle (25, -8) node[pos=0.5] {};
\fill[fill=gc_gray] (21, -8) rectangle (25, -9) node[pos=0.5] {};
\fill[fill=gc_blue] (21, -9) rectangle (25, -10) node[pos=0.5] {};
\fill[fill=gc_gray] (21, -10) rectangle (25, -11) node[pos=0.5] {};

% Empty Value Tensor
\fill[fill=none] (19.5, -1) rectangle (20.5, -2) node[pos=0.5] {\LARGE $\bm{V}_{[\textcolor{gc_dark_blue}{\bm{i}_2}, :]}$};
\filldraw[draw=black, fill=none] (21, -1) rectangle (25, -11) node[pos=0.5] {};
\draw (22, -1) to (22, -11);
\draw (23, -1) to (23, -11);
\draw (24, -1) to (24, -11);
\draw (21, -2) to (25, -2);
\draw (21, -3) to (25, -3);
\draw (21, -4) to (25, -4);
\draw (21, -5) to (25, -5);
\draw (21, -6) to (25, -6);
\draw (21, -7) to (25, -7);
\draw (21, -8) to (25, -8);
\draw (21, -9) to (25, -9);
\draw (21, -10) to (25, -10);


% Step 3
\draw[thick, -Triangle, color=black] (8.75, -11.7) -- (8.75, -12.6);
\fill[fill=none] (7.5, -11.5) rectangle (9, -16) node[pos=0.5] {\huge $\alpha=\displaystyle\sum_{\mathclap{i \in \textcolor{gc_dark_blue}{\bm{i}_2}}} \hat{s}_i$};


\filldraw[draw=black, fill=gc_dark_gray] (21, -12.5) rectangle (25, -13.5) node[pos=0.5] {};
\draw (22, -12.5) to (22, -13.5);
\draw (23, -12.5) to (23, -13.5);
\draw (24, -12.5) to (24, -13.5);

\draw [thick,decoration={brace,mirror,amplitude=10pt},decorate] (21, -13.75) -- (25, -13.75);
\fill[fill=none] (21, -14.75) rectangle (25, -14.25) node[pos=0.5] {\LARGE $\bm{\bar{v}}=\text{mean}(\bm{V})$};


\fill[fill=none] (26.5, -11.75) rectangle (26.5, -11.75) node[pos=0.5] {\LARGE $\bm{\oplus}$};
\draw[thick, -Triangle, color=black] (26.75, -11.75) -- (28.625, -11.75);
\fill[fill=none] (29, -11.75) rectangle (29, -11.75) node[pos=0.5] {\LARGE $\bm{y}$};

% Lines to the final addition
\draw[thick, color=black] (25, -13) -- (26.5, -13);
\draw[thick, -Triangle, color=black] (26.5, -13) -- (26.5, -12);

\draw[thick, color=black] (25, -2.5) -- (26.5, -2.5);
\draw[thick, color=black] (25, -3.5) -- (26.5, -3.5);
\draw[thick, color=black] (25, -6.5) -- (26.5, -6.5);
\draw[thick, color=black] (25, -9.5) -- (26.5, -9.5);
\draw[thick, -Triangle, color=black] (26.5, -2.5) -- (26.5, -11.5);

\fill[fill=none] (27.7, -12.75) rectangle (27.7, -12.75) node[pos=0.5] {\Large $\times\,(1-\alpha)$};
\fill[fill=none] (27.1, -10.75) rectangle (27.1, -10.75) node[pos=0.5] {\Large $\times\,\alpha$};

\end{tikzpicture}


==> tables/benchmarks_ipu.tex <==
\begin{tabular}{ c|c }
\textbf{Kernel} & \textbf{M2000 (1 Mk2 IPU)} \\\hline

%Baseline (local SRAM) & $134$ \us{} ($345\times$) \\\hline

Baseline & $40.4$ ms ($1\times$) \\

SparQ & $5.28$ ms ($7.7\times$) \\

\end{tabular}


==> tables/compression_ratios_table.tex <==
%auto-ignore

\begin{tabular}{ | c | c | c | c | }
\hline
 \textbf{Method} & $k$ & $r$ & \textbf{Compression} \\\hline

 \multirow{3}{*}{SparQ Attention}
 &\multirow{3}{*}{$128$}
 & $16$ & $0.13$ - $0.17$ \\\cline{3-4}
 & & $32$ & $0.19$ - $0.23$ \\\cline{3-4}
 & & $64$ & $0.31$ - $0.36$ \\\hline
 
 \multirow{5}{*}{H$_2$O}
 & $192$
 & \multirow{5}{*}{--} & $0.10$ - $0.17$ \\\cline{2-2}\cline{4-4}
 & $256$ & & $0.13$ - $0.22$ \\\cline{2-2}\cline{4-4}
 & $384$ & & $0.20$ - $0.33$ \\\cline{2-2}\cline{4-4}
 & $512$ & & $0.26$ - $0.43$ \\\cline{2-2}\cline{4-4}
 & $768$ & & $0.39$ - $0.65$ \\\hline
 
\end{tabular}

